The Geometry of Persona: Disentangling Personality from Reasoning in Large Language Models

Background: The deployment of personalized Large Language Models (LLMs) is currently constrained by the stability-plasticity dilemma. Prevailing alignment methods, such as Supervised Fine-Tuning (SFT), rely on stochastic weight updates that often incur an "alignment tax" -- degrading general reasoning capabilities. Methods: We propose the Soul Engine, a framework based on the Linear Representation Hypothesis, which posits that personality traits exist as orthogonal linear subspaces. We introduce SoulBench, a dataset constructed via dynamic contextual sampling. Using a dual-head architecture on a frozen Qwen-2.5 base, we extract disentangled personality vectors without modifying the backbone weights. Results: Our experiments demonstrate three breakthroughs. First, High-Precision Profiling: The model achieves a Mean Squared Error (MSE) of 0.011 against psychological ground truth. Second, Geometric Orthogonality: T-SNE visualization confirms that personality manifolds are distinct and continuous, allowing for "Zero-Shot Personality Injection" that maintains original model intelligence. Third, Deterministic Steering: We achieve robust control over behavior via vector arithmetic, validated through extensive ablation studies. Conclusion: This work challenges the necessity of fine-tuning for personalization. By transitioning from probabilistic prompting to deterministic latent intervention, we provide a mathematically rigorous foundation for safe, controllable AI personalization.

==> paper_assets/Table_1.tex <==

\begin{table}[h]
    \centering
    \caption{Performance Metrics on SoulBench Validation Set}
    \label{tab:metrics}
    \begin{tabular}{lcc}
        \toprule
        \textbf{Metric} & \textbf{Value (Best)} & \textbf{Value (Final)} \\
        \midrule
        MSE (Psychometric) & \textbf{0.0113} & 0.0118 \\
        Total Loss & - & 1.3184 \\
        \bottomrule
    \end{tabular}
\end{table}

